Distributed call-by-value machines

We present a new abstract machine, called DCESH, which describes the execution of higher-order programs running in distributed architectures. DCESH implements a generalised form of Remote Procedure Call that supports calling higher-order functions across node boundaries, without sending actual code. Our starting point is a variant of the SECD machine that we call the CES machine, which implements reduction for untyped call-by-value PCF. We successively add the features that we need for distributed execution and show the correctness of each addition. First we add heaps, forming the CESH machine, which provides features necessary for more efficient execution, and show that there is a bisimulation between the CES and the CESH machine. Then we construct a two-level operational semantics, where the high level is a network of communicating machines, and the low level is given by local machine transitions. Using these networks, we arrive at our final system, the distributed CESH machine (DCESH). We show that there is a bisimulation relation also between the CESH machine and the DCESH machine. All the technical results have been formalised and proved correct in Agda, and a prototype compiler has been developed.

==> dceshc-0.1.0.0/README <==
DCESH Compiler
==============
Author: Olle Fredriksson
Date: January 2014
License: See the LICENSE file

General information
-------------------
This is a compiler for a small untyped functional language, made to accompany
the paper "Distributed call-by-value machines". The compiler targets C and the
MPI library.

The compiler allows writing distributed programs with "locus specifiers":

  let f = (\x. x * x)@a in (f 3 + f 4)@b

This means that the function f is on node a and is called from node b. The
communication is handled automatically by the compiler and runtime system.

Compatibility
-------------
The compiler has been tested using the GHC compiler version 7.6.3 and the mpich
library version 3.0.4. Other versions may work too.

Installation
------------
Use cabal, which should come with e.g. the Haskell platform. In this directory,
run:

  > cabal install

This should create (by default in ~/.cabal/bin) a binary called dceshc.

Usage
-----
See the examples directory for some small examples. To compile an example, run:

  > dceshc example.lambda

This creates a directory 'out' in the same directory with a bunch of C files
(one for each node) and a Makefile.
To compile and run the program, do:

  > cd out
  > make DEBUG=y run

Making with DEBUG=y means that running the program prints some information
about what's happening in the execution (which may be out of order since it is
printing from several communicating processes). Making without the flag means
that it only prints the (assumed integer) result of the program, which is
perhaps less exciting.

